The Graph Pencil Method: Mapping Subgraph Densities to Stochastic Block Models

In this work, we describe a method that determines an exact map from a finite set of subgraph densities to the parameters of a stochastic block model (SBM) matching these densities. Given a number $K$ of blocks, the subgraph densities of a finite number of stars and bistars uniquely determines a single element of the class of all degree-separated stochastic block models with $K$ blocks. Our method makes it possible to translate estimates of these subgraph densities into model parameters, and hence to use subgraph densities directly for inference. The computational overhead is negligible; computing the translation map is polynomial in $K$, but independent of the graph size once the subgraph densities are given.

==> 031relatedwork.tex <==
\section{Related Work}
\label{sec:RelatedWork}


% Other works on matrix/tensor methods for recovering models of distributions over graphs
% \cite{anandkumar2013tensor}

% \begin{itemize}
%     \item Variational Bayes model averaging for graphon functions and motif frequencies inference in W-graph models \cite{latouche2016variational}
% \end{itemize}

% \paragraph{Matrix pencil method}
% % \label{ssec:RelatedProny}
% \begin{itemize}
%    \item Method of moments 
%     \item Prony's method \cite{sauer2018prony, prony1795essai}
%     \item Renewed theoretical interest in this type of models -- eg, COLT2021 source identification for mixture of discrete product distributions \cite{gordon2021source} 
%     \item Matrix pencil 
%     \item Compressed sensing \cite{candes2006stable}
% \end{itemize}

% Bickel \cite{bickel2011method}

% \paragraph{The Method of Moments}

==> 040overview.tex <==
\section{Overview}
\label{sec:Overview}

The rest of our paper is organized as follows: \\
% The heart of our paper is organized as follows: % meat 
In section~\ref{sec:ProblemSetUpAndNotation}, we provide the notation and basic definitions. \\
We then explain how to recover the parameters of a SBM given a set of subgraph densities, without worrying about how to estimate those densities from data (section~\ref{sec:DataToSBM}). 
To this end, we first describe how to apply the standard  {\classicalmethodnameM} to infer the parameters of a Bernoulli mixture model (section~\ref{SI:MixtureModel}).
We then show how the same procedure can be used to recover 
the normalized degrees of the latent {\latentnodes} 
(and thereby also their proportions) of an SBM, and why the method works. 
This procedure is the first step of the proposed {\ourmethodnameM}.
We then describe how to obtain the parameters for the connection of the different types of edges (section~\ref{sec:GettingtheBmatrix})...\\
% \ref{sec:GettingtheBmatrix}
% \ref{sec:GluingGraphs}
% \ref{sec:AddingMoreSubgraphs}
% \ref{sec:SymmetricSBM}

% In section~\ref{sec:DataToSBM}, we describe how to infer  real data. 
% Tootsie-roll subgraphs. 
% In Section~\ref{sec:DataToSBM}
% \ref{sec:subgraphcount}
% \ref{ssec:tootsierollcounts}

% We conclude with simulations (section~\ref{sec:Experiments}) and discussion (section~\ref{sec:Discussion}).
% \ref{sec:RelatedWork}












==> 070themethodAlgorithm.tex <==
% \begin{algorithm}[ht]
% \caption{Shannon entropy estimation for tree-structured distribution \label{alg:fastmst}}
% \begin{algorithmic}[1]
% \State Let ...
% % $M = \left\lceil \frac{2}{\eps} \right\rceil$ and $R = \left\lceil \frac{1}{\eps^2} \right\rceil$
% \For{$m = 1, \ldots, M$}
% \For{$r = 1, \ldots, R$}
% \State Choose positive integer $Z$ randomly according to $\Pr[Z \ge z] = 1 / z$.
% \State Choose $i^*$ uniformly at random from $[d]$.
% \If{$Z \ge \frac{2}{\eps}$} $\;\gamma_{mr} \gets 0$.
% \Else \Comment{Breadth-first search}
% \State Initialize queue to contain $i^*$ and a set $V=\{i^*\}$.
% \While{queue length is non-zero and shorter than $Z$}
% \State Remove $i$ from front of queue and $V = V\cup \{i\}$.
% \For{$j = [d] \setminus V$}
% \State Server computes $(\alpha, \eps, \delta)$-good estimate $\hI_{ij}$ of $I(X_i; X_j)$.
% \If{$\hI_{ij} \ge \eps m$} add $j$ to back of queue.
% \EndIf
% \EndFor
% \EndWhile
% \If{queue length is zero} $\gamma_{mr} \gets 0$ {\bf else} $\gamma_{mr} \gets 1$.
% \EndIf
% \EndIf
% \EndFor
% \State $\;\hc_m \gets \frac{d}{R} \sum_{r=1}^R \gamma_{mr}$.
% \EndFor
% \State $\hat{W} \gets \epsilon Md - \epsilon\sum_{m=1}^M \hc_m$
% % \State Server computes $(\alpha, \eps, \delta)$-good estimate of each entropy in the first sum in Eq.~\eqref{eq:clmain}.
% \State Let $\hat{S}$ be the sum of the entropy estimates.
% \State Return $\hH = \hat{S} - \hat{W}$.
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
    \caption{Euclid’s algorithm}
    \label{euclid}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        \Procedure{Euclid}{$a,b$} \Comment{The g.c.d. of a and b}
            \State $r\gets a \bmod b$
            \While{$r\not=0$} \Comment{We have the answer if r is 0}
                \State $a \gets b$
                \State $b \gets r$
                \State $r \gets a \bmod b$
            \EndWhile\label{euclidendwhile}
            \State \textbf{return} $b$\Comment{The gcd is b}
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> 080experiments.tex <==
\section{Experiments}
\label{sec:Experiments}

We show simulations In Appendix~\ref{SI:Experiments}. 

% \subsection{Synthetic Data}
% Convergence:
% \begin{itemize}
%     % \item Toy problem: 2x2, equal communities, positive clustering, positive degree heterogeneity
%     \item Two curves per plot, one large degree separation, one small (maybe a third)
%     \item Plot accuracy of pentagon (square and triangle too?) density
%     \item As a function of number of nodes in the graph
%     \item Do one with constant edge density, one with constant expected degree
% \end{itemize}
% Parameter selection:
% \begin{itemize}
%     \item Same as above (but maybe with a 3x3)
%     \item Show convergence curves for k-1, k and k+1
% \end{itemize}

% \begin{itemize}
% \item having two plots one for dense regime and for sparse regime 
% \item a plot for k-ssbm recover
% \item  subgraphs used in the inference and their densities in the inferred distribution (for a large-ish k-sbm)
% \end{itemize}




% \subsection{Real-world Data}
% \begin{itemize}
%     \item french political blogsphere network (196 vertices and 2864 edges) [compare with the results from \cite{latouche2016variational}]
% \end{itemize}

==> intro-porbanz.tex <==
It is well-known that every distribution of an infinite exchangeable graph is completely determined by
all subgraph densities of finite subgraphs \citep{Diaconis:Janson:2007,lovasz2012large}. This class of distributions
contains all graphon models and stochastic block models \citep{Diaconis:Janson:2007}. 
The subgraph densities can be regarded as the graph equivalent to the moments of classical statistical inference \citep{Bickel:Chen:Levina:2011}. 
It is possible to estimate a single subgraph density,
or a finite number of them, consistently and at a guaranteed asymptotic rate from a single data
graph as the graph grows large \citep{Bickel:Chen:Levina:2011,Ambroise:Matias:2012}.
Estimating these densities, however, is only a first step in the inference process, and there is no
general way of translating them into an estimate of a graphon or stochastic block model. 
% Instead,
% most inference algorithms used in practice rely on some combination of MCMC sampling, variational inference \cite{celisse2012consistency,latouche2016variational}, clustering of the nodes, or other heuristics.
Instead,
most inference algorithms used in practice rely on some combination of MCMC sampling, variational inference \cite{celisse2012consistency,latouche2016variational}, clustering of the nodes, or other heuristics.

This paper solves several problems simultaneously: efficiently estimate parameters without laborious and delicate numerical
fitting, and efficiently sampling from the model without the well-documented issue of degeneracy \cite{lauritzen2018random,Gunderson2019Introducing}.
To this end, we generalize a method for i.i.d.\ samples, sometimes known as Prony's method \cite{prony1795essai}, to graph data.
The classical Prony's method is an example of an algorithm that recovers a sparse signal from a very small number of
samples, and has is related to compressed sensing [ADD CITATION TO SAUER (?) PAPER].
Our generalization of this method to graphs is related to the idea of a matrix pencil \citep{Markus:1988}.
[NAME PROPERTIES WE CAN ESTIMATE, ADD A FEW MORE WORDS ON GLYPH ALGEBRA, MAYBE ON THE METHOD BEING STABLE DESPITE USING VANDERMONDE MATRIX ETC]

The method proceeds in two steps.  
The first step is essentially an application of the classical Prony's method to estimate properties of individual latent communities, 
such as their normalized degrees and their relative sizes.  
The second step is entirely new; by leveraging the properties inferred in the first step, it uses a generalization of Prony's method to infer properties of \textit{pairs} of the latent communities, such as the connection properties of a stochastic block model.  

Moreover, the method is able to incorporate additional subgraph densities.  
We show that this flexibility allows it to be applied in situations where other 



% @book{Markus:1988,
%   author={Markus, A.~S.},
%   title={Introduction to the Spectral Theory of Polynomial Operator Pencils},
%   publisher={American Mathematical Society},
%   year=1988}

% @article{Diaconis:Janson:2007,
% 	Author = {P. Diaconis and S. Janson},
% 	Journal = {Rendiconti di Matematica, Serie VII},
% 	Keywords = {graphs},
% 	Pages = {33--61},
% 	Title = {Graph limits and exchangeable random graphs},
% 	Volume = {28},
% 	Year = {2008}}

% @article{Bickel:Chen:Levina:2011:1,
% 	Author = {P.~J. Bickel and A. Chen and E. Levina},
% 	Journal = {Ann. Statist.},
% 	Number = {5},
% 	Pages = {2280--2301},
% 	Title = {The method of moments and degree distributions for network models},
% 	Volume = {39},
% 	Year = {2011}}

% @article{Ambroise:Matias:2012:1,
% 	Author = {Ambroise, C. and Matias, C.},
% 	Journal = {J.\ R.\ Stat.\ Soc.\ Ser.\ B.},
% 	Pages = {3--35},
% 	Title = {New consistent and asymptotically normal parameter estimates for random-graph mixture models},
% 	Volume = {74},
% 	Year = {2012}}



==> notFornowUnbiasingMatrixPencil.tex <==
\section{Improving the Matrix Pencil} 

\subsection{Scaling by the precision} 

\subsubsection{Estimating the variance} 
\label{ssec:variance}
We can estimate this using a sort of jackknife estimator.  
In contrast to typical implementations, we can do this without incurring additional computational cost.  
For each node, we can count the number of injective homomorphism counts are removed if that node were deleted.  
Then we can use the distribution of these counts to estimate the variance of that subgraph density:
\begin{align}
    \mathrm{Var}\big(\mu_g^{ }(G)\big) \approx \frac{n}{n-1}\sum_{i=1}^n \Big(\mu_g^{ }(G\setminus i) - \mu_g^{ }(G) \Big)^{\kern-1pt2}_{ }
\end{align}
For each node, we already have the number of counts for which it is one of the center nodes of the subgraph.  
For the counts where it is one of the neighboring nodes, 
we can use the same ideas as before, computing the estimator exactly without increasing computational cost.  

To verify the correctness of these expressions, 
we take a generic SBM and simulate multiple graphs with $n$ nodes, 
and compare the variance of the observed distribution of subgraph densities with the distribution of the estimated variances.  

\begin{itemize}
    \item Give an idea of the error in the approximation of the variance 
    \item Give an idea of magnitude of the improvement 
    % \item Discussion of what subgraphs to include
\end{itemize}

\subsection{Using more orthogonal linear combinations} 

==> oldtext.tex <==
% \section{Classical Case: Bernoulli Mixture Model} %Exchangeable Binary Sequences}
% \label{SI:MixtureModel}

% % \GBH{Mixture models are an effective way to build more complicated distributions from simpler distributions by introducing latent variables that }
% % An alternative to maximum likelihood and EM, especially in the context of mixture
% % models, is the method of moments approach. The method of moments dates back to the
% % origins of mixture models with Pearson’s solution for identifying the parameters of a mixture
% % of two univariate Gaussians (Pearson, 1894). In this approach, model parameters are chosen
% % to specify a distribution whose p-th order moments, for several values of p, are equal to the corresponding empirical moments observed in the data. S
% % a number of
% % moment methods for both discrete and continuous mixture models have been developed
% % using techniques such as the Vandermonde decompositions of Hankel matrices (Lindsay,
% % 1989; Lindsay and Basak, 1993; Boley et al., 1997; Gravin et al., 2012). In these methods,
% % following the spirit of Pearson’s original solution, the model parameters are derived from the
% % roots of polynomials whose coefficients are based on moments up to the Ω(k)-th order.

% Consider the well-studied Bernoulli mixture model (aka, the $k$-coin model),  
% % $\mathcal{M}(b_k, \pi_k)$, 
% % which describes all infinite sequences of binary random variables that are exchangeable. 
% % where a sequence of binary outcomes 
% % describing the resulting of sampling from a pile of 
% % describing the exchangeable binary sequences induced by the outcome of flips of coins sampled i.i.d. from an opaque bag containing an infinite supply of a (possibly unequal) mixture of $K$ different types of biased coins, i.e, each coin of type $k\in[K]$ has bias \mbox{$b_k^{ }\in[0,1]$} to come up heads.
% % with describes all exchangeable binary sequences. 
% which describes exchangeable sequences of binary variables. 
% These can be thought of as the outcomes of flips of coins sampled iid from an opaque bag with an infinite supply of a (possibly unequal) mixture of $K$ different types of biased coins, ie, all coins of type $k\in[K]$ have the same bias \mbox{$b_k^{ }\in[0,1]$} to come up heads.
% % describing all exchangeable binary sequences induced by the outcome of flips of coins sampled i.i.d. from an opaque bag with an infinite supply of a (possibly unequal) mixture of $K$ different types of biased coins, i.e, each coin of type $k\in[K]$ has bias \mbox{$b_k^{ }\in[0,1]$} to come up heads.
% % describing the exchangeable binary sequences induced by the outcome of flips of coins sampled i.i.d. from an opaque never-ending bag of coins containing a (possibly unequal) mixture of $K$ different types of biased coins, i.e, each coin of type $k\in[K]$ has bias \mbox{$b_k^{ }\in[0,1]$} to come up heads.
% % induced by sampling i.i.d. from an opaque never-ending bag of coins containing a (possibly unequal) mixture of $K$ different types of biased coins, i.e, each coin of type $k\in[K]$ has bias \mbox{$b_k^{ }\in[0,1]$} to come up heads.
% Both the fraction \mbox{$\pi_k^{ }$} of coins of type \mbox{$k\in[K]$} as well as their bias \mbox{$b_k^{ }\in[0,1]$} are not observable. 
% %
% % , where each type \mbox{$k\in[K]$} has a (different) bias \mbox{$b_k^{ }\in[0,1]$} to come up heads, but you do not know how many coins there are of each type, nor their biases.  
% % resulting from sampling from a (arbitrary large) pile of $K$ types of biased coins, where each type has a (different) bias to come up heads, but you do not know how many coins there are of each type, nor their biases.  

% The $r^{\text{th}}_{ }$ moment (where $r$ is a nonnegative integer) of this distribution is: 
% \begin{align}
% % \mu_r^{ } = \sum_k^{ } \pi_k^{ } b_k^r \label{Eq:Moments}
% \langle b^r_{ }\rangle = \sum_k^{ } \pi_k^{ } b_k^r \label{Eq:Moments}
% \end{align}
% % A Matrix Pencil method offers a way to systematically infer $\vecttsymbol{\pi}$ and $\vectt{b}$ from these moments. 
% The mixture proportion $\vecttsymbol{\pi}$ and the biases $\vectt{b}$ can be systematically inferred from these moments using a Matrix Pencil/generalized Prony's method. % Matrix Pencil method. 
% In particular, 
% let \mbox{$M_{i\!j}^{ } = \mu_{i+j}^{ }$} and \mbox{$M'_{i\!j} = \mu_{i+j+1}^{ }$} be the following %\mbox{$K\times K$} 
% Hankel\footnote{A Hankel matrix is a symmetric square matrix with constant positive-sloping skew-diagonals.} matrices:
% % A diagonal of a square matrix which is traversed in the "northeast" direction. "The" skew diagonal (or "secondary diagonal") of an n×n square matrix is the skew diagonal from a_(n1) to a_(1n).

% \begin{align*}
% \matt{M} = \left[
%     \begin{array}{llll}
%     \langle b^0_{ }\rangle   &   \langle b^1_{ }\rangle   &   \cdots   &   \langle b^{K-1}_{ }\rangle\\
%     \langle b^1_{ }\rangle   &   \langle b^2_{ }\rangle   &   \cdots   &   \langle b^{K}_{ }\rangle   \\
%     \vdots   &   \vdots   &    \ddots   &   \vdots\\
%     \langle b^{K-1}_{ }\rangle   &   \langle b^{K}_{ }\rangle   &   \cdots   &   \langle b^{2K-2}_{ }\rangle\\
%     \end{array}
%     \right]\kern24pt 
% \matt{M'} = \left[
%     \begin{array}{llll}
%     \langle b^1_{ }\rangle   &   \langle b^2_{ }\rangle   & \cdots   &   \langle b^K_{ }\rangle   \\
%     \langle b^2_{ }\rangle   &   \langle b^3_{ }\rangle   &   \cdots   &   \langle b^{K+1}_{ }\rangle   \\
%     \vdots   &   \vdots   &    \ddots   &   \vdots\\
%     \langle b^K_{ }\rangle   &   \langle b^{K+1}_{ }\rangle   &   \cdots   &   \langle b^{2K-1}_{ }\rangle   \\
%     \end{array}
%     \right],
% \end{align*}
% % as we will show in the next section, 
% the eigenvalues of \mbox{$\matt{M'}\matt{M}^{-1}_{ }$} are the entries of $\vectt{b}$, 
% and from those the associated entries of $\vecttsymbol{\pi}$ can be straightforwardly obtained.  

% \section{Getting Graphical: Distilling the Degree Distribution}
% \label{SI:GettingDegreeDistribution}
% %
% % \GBHcomment{The first step of our proposed Graphical Matrix Pencil method is to apply this standard Matrix Pencil method to the obtain the (normalized) degrees $d_k^{ }$ of the communities:\\ -- connect with edge density/def}  

% The first step of the Graphical Matrix Pencil method is to apply this standard Matrix Pencil method to the obtain the (normalized) degrees $d_k^{ }$ of the communities:  
% % \GBH{The first step of the Graphical Matrix Pencil method is to apply this standard Matrix Pencil method to obtain the vector of community sizes, as well as, the (normalized) degrees $d_k^{ }$ of the communities}
% % $d_i^{ }$ and the community sizes $\pi_i^{ }$.  
% % First, we obtain the (normalized) degrees of the communities
% \begin{align}
% % \vectt{d} = \matt{W}\cdot\vectt{\pi}
% d_k^{ } = \sum_j^{ } \pi_j^{ } B_{jk}^{ }
% \end{align}
% %
% The moments of this distribution are indexed as in \eqref{Eq:Moments}:
% \begin{align}
% \mu_r^{ } = \sum_k^{ } \pi_k^{ } d_k^{r} \label{Eq:StarAlgebraicMoments}
% \end{align}
% To see why the method works, notice that the Hankel matrices are a sum of \mbox{rank-1} matrices (weighted by \mbox{$\pi_k^{ }$}), and thus can be diagonalized as follows: 
% \begin{align}
% \matt{M} &= %\left[
%     % \begin{array}{cccc}
%     % \mu_0^{ }   &   \mu_1^{ }   &   \cdots&   \mu_{K-1}^{ }   \\
%     % \mu_1^{ }   &   \mu_2^{ }   &   \cdots&   \mu_K^{ }   \\
%     % \vdots   &   \vdots   &   \ddots&   \vdots   \\
%     % \mu_{K-1}^{ }   &   \mu_K^{ }   &   \cdots   &   \mu_{2K-2}^{ }\\
%     % \end{array}
%     % \right] = 
%     \sum_k^{ } \pi_k^{ } \left[
%     \begin{array}{cccc}
%     d_k^{0}   &   d_k^{1}   &   \cdots   &   d_k^{K-1}\\
%     d_k^{1}   &   d_k^{2}   &   \cdots   &   d_k^{K}\\
%     \vdots   &   \vdots   &   \ddots   &   \vdots\\
%     d_k^{K-1}   &   d_k^{K}   &   \cdots   &   d_k^{2K-2}\\
%     \end{array}
%     \right] = \sum_k^{ } \pi_k^{ } \left[
%     \begin{array}{c}
%     d_k^{0}   \\
%     d_k^{1}   \\
%     \vdots   \\
%     d_k^{K-1}   \\
%     \end{array}
%     \right]  \left[
%     \begin{array}{c}
%     d_k^{0}   \\
%     d_k^{1}   \\
%     \vdots   \\
%     d_k^{K-1}   \\
%     \end{array}
%     \right]^\transpose \\
% &= \left[
%     \begin{array}{cccc}
%     d_1^{0}   &   d_2^{0}   &   \cdots   &   d_K^{0}\\
%     d_1^{1}   &   d_2^{1}   &   \cdots   &   d_K^{1}\\
%     \vdots   &   \vdots   &   \ddots   &   \vdots\\
%     d_1^{K-1}   &   d_2^{K-1}   &   \cdots   &   d_K^{K-1}\\
%     \end{array}
%     \right]\left[
%     \begin{array}{cccc}
%     \pi_1^{ }   &   0   &   \cdots  &   0   \\
%     0   &   \pi_2^{ }   &   \cdots  &   0   \\
%     \vdots   &   \vdots   &   \ddots   &   \vdots\\
%     0   &   0   &   \cdots   &   \pi_K^{ }\\
%     \end{array}
%     \right]\left[
%     \begin{array}{cccc}
%     d_1^{0}   &   d_2^{1}   &   \cdots   &   d_K^{K-1}\\
%     d_2^{0}   &   d_3^{1}   &   \cdots   &   d_K^{K-1}\\
%     \vdots   &   \vdots   &   \ddots   &   \vdots\\
%     d_K^{0}   &   d_{K+1}^{1}   &   \cdots   &   d_K^{K-1}\\
%     \end{array}
%     \right]\\
%     &= \matt{V} \text{ diag$(\vecttsymbol{\pi})$ } \matt{V}^\transpose
%     \end{align}
% % where $V_{jk}^{ } = d_k^{j-1}$ is the (Vandermonde) matrix of powers of the degrees: 
% where \mbox{$V_{jk}^{ } = d_k^{j-1}$} is the Vandermonde\footnote{A Vandermonde matrix is a matrix with terms of a geometric progression in each column.} matrix of powers of the degrees: 
% \begin{align}
% \matt{V} = \left[
%     \begin{array}{cccc}
%     d_1^{0}   &   d_2^{0}   &   \cdots   &   d_K^{0}\\
%     d_1^{1}   &   d_2^{1}   &   \cdots   &   d_K^{1}\\
%     \vdots   &   \vdots   &   \ddots   &   \vdots\\
%     d_1^{K-1}   &   d_2^{K-1}   &   \cdots   &   d_K^{K-1}\\
%     \end{array}
%     \right]
% \end{align}
% By the same decomposition, we also have:  
%     \begin{align}
% \matt{M'} %&= \left[
%     % \begin{array}{cccc}
%     % d_1^{0}   &   d_2^{0}   &   \cdots   &   d_K^{0}\\
%     % d_1^{1}   &   d_2^{1}   &   \cdots   &   d_K^{1}\\
%     % \vdots   &   \vdots   &   \ddots   &   \vdots\\
%     % d_1^{K-1}   &   d_2^{K-1}   &   \cdots   &   d_K^{K-1}\\
%     % \end{array}
%     % \right]\left[
%     % \begin{array}{cccc}
%     % \pi_1^{ }d_1^{ }   &   0   &   \cdots   &   0\\
%     % 0   &   \pi_2^{ }d_2^{ }   &   \cdots   &   0\\
%     % \vdots   &   \vdots   &   \ddots&   \vdots   \\
%     % 0   &   0   &   \cdots&   \pi_K^{ }d_K^{ }   \\
%     % \end{array}
%     % \right]\left[
%     % \begin{array}{cccc}
%     % d_1^{0}   &   d_1^{1}   &   \cdots&   d_1^{K-1}   \\
%     % d_2^{0}   &   d_2^{1}   &   \cdots&   d_2^{K-1}   \\
%     % \vdots   &   \vdots   &   \ddots    &   \vdots   \\
%     % d_K^{0}   &   d_K^{1}   &   \cdots  &   d_K^{K-1}   \\
%     % \end{array}
%     % \right]\\
%     &= \matt{V} \text{ diag$(\vecttsymbol{\pi} \vectt{d})$ } \matt{V}^\transpose
% \end{align}
% %
% The eigendecomposition of \mbox{$\matt{M}'\matt{M}^{-1}_{ }$} is now clear:
% \begin{align}
%     \matt{M}'_{ }\matt{M}^{-1}_{ } &= \big(\matt{V}\text{ diag$(\vecttsymbol{\pi} \vectt{d})$ }\matt{V}^{\transpose}_{ }\big)\big(\matt{V}\text{ diag$(\vecttsymbol{\pi}_{ }^{ })$ }\matt{V}^{\transpose}_{ }\big)^{-1}_{ } \\
%     &= \matt{V}\text{ diag$(\vecttsymbol{\pi} \vectt{d})$ }\matt{V}^{\transpose}_{ }\big(\matt{V}^\transpose_{ }\big)^{-1}_{ }\text{ diag$(\vecttsymbol{\pi}_{ }^{-1})$ }\matt{V}^{-1}_{ } \\
%     &= \matt{V}\text{ diag$(\vecttsymbol{\pi} \vectt{d})$  diag$(\vecttsymbol{\pi}_{ }^{-1})$ }\matt{V}^{-1}_{ } \\
%     &= \matt{V}\text{ diag$(\vectt{d})$ }\matt{V}^{-1}_{ } 
% \end{align}
% %
% % The eigendecomposition of \mbox{$\matt{M}'\matt{M}^{-1}_{ }$} is now clear:
% And so our solution can be written as: 
% \begin{align}
%     \text{eigval}\Big(\matt{M}'_{ }\matt{M}^{-1}_{ }\Big) &= \vectt{d} \\
%     \text{eigvec}\Big(\matt{M}'_{ }\matt{M}^{-1}_{ }\Big) &= \matt{V} \\
%     % \matt{V}^{-1}_{ }\vecttsymbol{\mu } &= \vecttsymbol{\pi}
%     \matt{V}^{-1}_{ }\vecttsymbol{\langle d^\star \rangle} &= \vecttsymbol{\pi}
% \end{align}
% % % Clearly, by selecting one coin and flipping it many times, it is possible to estimate the bias $b$ of one of the types.  
% % You sample $n$ coins iid from the pile, and flip each $m$ times.  
% %
% Notice that this procedure relies on the fact that the degrees of the communities are unique, otherwise $\matt{V}$ will not be invertible.  


% \subsection{The Graphical Matrix Pencil Method: Extracting the Edge Expectations}

% The previous matrices $\matt{M}$ and $\matt{M}'$ were obtained by summing once over the $K$ communities. 
% This allowed us to obtain properties related to a single community.  %, such as their (normalized) degrees $\vectt{d}$).  
% The first main insight of this paper is that the matrix pencil method can be extended to obtain the entries of $\matt{B}$, the connection probabilities between pairs of communities.  

% At this point, it is useful to introduce our notation for rooted subgraphs.  
% A subgraph of a graph $G$ is a set of vertices of $G$ and a (possibly proper) subset of the edges connecting these vertices in $G$.  
% A rooted subgraph is a subgraph combined with (ordered) list of one or more vertices in this subgraph. These vertices are called roots.  

% \LMG{what a rooted subgraph means, loop over k for each rooted node, so indicates the density of the subgraph when those rooted nodes are in those particular communities}
% % To do so, the sums over \mbox{$k\leq K$} must be replaced with sums over the $\frac{1}{2}K(K+1)$ pairs \mbox{$i\leq j\leq K$}.  
% Rooted nodes are denoted by open circles, and computationally represent a vector of ones: \LMG{vector of length k, what it means...}
% \begin{align}
% \text{(rooted node)} \kern6pt \OpenNodeOld &\longleftrightarrow \vecttsymbol{1} \kern9pt \text{(vector of ones)}
% % \end{align}
% \intertext{Algebraically, this is the identity for entrywise multiplication (aka the ``gluing'' product, or Hadamard product).  
% Given two rooted subgraphs, 
% the gluing product is obtained by taking their disjoint union, 
% then identifying the two rooted nodes.  
% %, which is denoted by the intentionally similar symbol $\circ$.  Computationally, the gluing operation is simply entrywise multiplication.  
% As it should, gluing the identity with the identity yields the identity.  
% To make things more interesting, let us attach an edge to the rooted node.  
% Computationally, this is the vector of the normalized degrees of the $K$ communities:}  %\footnote{For now, this is a vector of the $K$ normalized degrees.}
% % \begin{align}
% \text{(rooted edge)} \kern6pt \OpenNodeOldEdge &\longleftrightarrow \vectt{d} \kern9pt \text{(vector of degrees)}\\
% % \end{align}
% \intertext{Gluing it with itself gives}
% % \begin{align}
% \text{(gluing rooted nodes)} \kern6pt \OpenNodeOldEdge \circ \OpenNodeOldEdge = \OpenNodeOldTwoEdge &\longleftrightarrow \vectt{d}^{ }_{ } \circ \vectt{d}^{ }_{ } = \vectt{d}^{2}_{ } \kern9pt \text{(entrywise multiplication)}%\\
% % \OpenNodeOldThreeEdge &\longleftrightarrow \vectt{d}^{ }_{ } \circ \vectt{d}^{2}_{ } = \vectt{d}^3_{ }
% \intertext{%and so on.  
% Taking the dot product of these vectors with $\vecttsymbol{\pi}$ corresponds to ``unrooting'' the rooted node.  }%The result is the density of the  
% % \begin{align}
% \text{(unrooting rooted nodes)} \kern6pt \ClosedNodeOldThreeEdge &\longleftrightarrow \vectt{d}^3_{ } \bullet \vecttsymbol{\pi} = \mu_3^{ }\kern9pt \text{(dot product)}
% \end{align}
% So c

% % \begin{center}
% % \begin{tabular}{ r c l }
% % rooted node & $\longleftrightarrow$ & vector of ones \\
% % gluing rooted nodes & $\longleftrightarrow$ & entrywise multiplication \\
% % unrooting a rooted node & $\longleftrightarrow$ & weighted sum over communities \\
% % \end{tabular}
% % \end{center}




% % \begin{center}
% % \begin{tabular}{ c l l }
% %  glyph & symbol & meaning \\ 
% %  \hline
% %  \OpenNodeOld & $1_i^{ }$ & vector of ones of length $k$\\  
% %  % \ClosedNodeOld & $\pi_i^{ }$ & vector of the $k$ community sizes \\  
% %  \OpenNodeOldEdge & $d_i^{ } = W_{i\!j}^{ } \pi_j^{ }$ & vector of the $k$ normalized degrees  \\
% %  \OpenNodeOldTwoEdge & $d_i^{2}$ & \\
% %  \vdots 
% % \end{tabular}
% % \end{center}



% \newpage
% drafts...  
% \newpage

% % \section{Distilling the Degree Distribution}
% % The first step of the Graphical Matrix Pencil method is to apply this standard Matrix Pencil method to the obtain the (normalized) degrees $d_i^{ }$ of the communities:  
% % % $d_i^{ }$ and the community sizes $\pi_i^{ }$.  
% % % First, we obtain the (normalized) degrees of the communities
% % \[
% % % \vectt{d} = \matt{W}\cdot\vectt{\pi}
% % d_i^{ } = \sum_j^{ } B_{i\!j}^{ }\pi_j^{ }
% % \]
% % % This is done using the classical method of Prony.  
% % % Essentially, treat the (normalized) degrees of individual nodes as iid samples from a mixture distribution.  
% % Essentially, treat the (normalized) degrees of individual nodes as i.i.d. samples from a mixture distribution.  

% % Consider the \mbox{$k$-by-$k$} (Hankel) matrix $M_{i\!j}^{ }$, where the ${i\!j}^\text{th}_{ }$ entry is given by the density of the subgraph with \mbox{$i+j$} edges meeting at a single node (the ``star'' subgraphs).  
% % For example, for \mbox{$k=3$}: 
% % \begin{align*}
% %     M_{i\!j}^{ } = \left[
% %     \begin{array}{ccc}
% %     1   &   \Edge   &   \Wedge   \\
% %     \Edge   &   \Wedge   &   \Claw   \\
% %     \Wedge   &   \Claw   &   \Cross
% %     \end{array}
% %     \right]
% % \end{align*}
% % This matrix can be decomposed into a sum over the $k$ communities: 
% % \begin{align}
% %     M_{i\!j}^{ } = \sum_k^{ } \pi_k^{ }
% %     \left[
% %     \begin{array}{ccc}
% %     d_k^{0}   &   d_k^{1}   &   d_k^{2}   \\
% %     d_k^{1}   &   d_k^{2}   &   d_k^{3}   \\
% %     d_k^{2}   &   d_k^{3}   &   d_k^{4}
% %     \end{array}
% %     \right]
% %     \label{Eq:MDegreeOuterProductSum}
% % \end{align}
% % or equivalently as a diagonal matrix sandwiched between two (Vandermonde)\footnote{A Vandermonde matrix has the terms of a geometric progression in each row.} matrices of the community degrees:
% % \begin{align*}
% %     \left[
% %     \begin{array}{ccc}
% %     1   &   1   &   1   \\
% %     d_1^{ }   &   d_2^{ }   &   d_3^{ }   \\
% %     d_1^{2}   &   d_2^{2}   &   d_3^{2}
% %     \end{array}
% %     \right]\left[
% %     \begin{array}{ccc}
% %     \pi_1^{ }   &   0   &   0   \\
% %     0   &   \pi_2^{ }   &   0   \\
% %     0   &   0   &   \pi_3^{ }
% %     \end{array}
% %     \right]\left[
% %     \begin{array}{ccc}
% %     1   &   d_1^{ }   &   d_1^{2}   \\
% %     1   &   d_2^{ }   &   d_2^{2}   \\
% %     1   &   d_3^{ }   &   d_3^{2}
% %     \end{array}
% %     \right]
% % \end{align*}
% % Now construct another matrix $M'_{i\!j}$, where the ${i\!j}^\text{th}_{ }$ entry is given by the density of the star subgraph with \mbox{$i+j+1$} edges:
% % \begin{align*}
% %     M'_{i\!j} = \left[
% %     \begin{array}{ccc}
% %     \Edge   &   \Wedge   &  \Claw\\
% %     \Wedge   &   \Claw   &   \Claw   \\
% %     \Claw  &   \Cross   &   \FiveStar
% %     \end{array}
% %     \right]
% % \end{align*}
% % This can also be decomposed as: 
% % \begin{align*}
% %     M'_{i\!j} = \sum_k^{ } \pi_k^{ }d_k^{ }
% %     \left[
% %     \begin{array}{ccc}
% %     d_k^{0}   &   d_k^{1}   &   d_k^{2}   \\
% %     d_k^{1}   &   d_k^{2}   &   d_k^{3}   \\
% %     d_k^{2}   &   d_k^{3}   &   d_k^{4}
% %     \end{array}
% %     \right]=\left[
% %     \begin{array}{ccc}
% %     1   &   1   &   1   \\
% %     d_1^{ }   &   d_2^{ }   &   d_3^{ }   \\
% %     d_1^{2}   &   d_2^{2}   &   d_3^{2}
% %     \end{array}
% %     \right]\left[
% %     \begin{array}{ccc}
% %     \pi_1^{ }d_1^{ }   &   0   &   0   \\
% %     0   &   \pi_2^{ }d_2^{ }   &   0   \\
% %     0   &   0   &   \pi_3^{ }d_3^{ }
% %     \end{array}
% %     \right]\left[
% %     \begin{array}{ccc}
% %     1   &   d_1^{ }   &   d_1^{2}   \\
% %     1   &   d_2^{ }   &   d_2^{2}   \\
% %     1   &   d_3^{ }   &   d_3^{2}
% %     \end{array}
% %     \right]
% % \end{align*}
% % When all $k$ degrees are different, these matrices are invertible.  The second matrix times the inverse of the first is
% % \begin{align*}
% %     M'_{ }M^{-1}_{ } = \left[
% %     \begin{array}{ccc}
% %     1   &   1   &   1   \\
% %     d_1^{ }   &   d_2^{ }   &   d_3^{ }   \\
% %     d_1^{2}   &   d_2^{2}   &   d_3^{2}
% %     \end{array}
% %     \right]\left[
% %     \begin{array}{ccc}
% %     d_1^{ }   &   0   &   0   \\
% %     0   &   d_2^{ }   &   0   \\
% %     0   &   0   &   d_3^{ }
% %     \end{array}
% %     \right]\left[
% %     \begin{array}{ccc}
% %     1   &   d_1^{ }   &   d_1^{2}   \\
% %     1   &   d_2^{ }   &   d_2^{2}   \\
% %     1   &   d_3^{ }   &   d_3^{2}
% %     \end{array}
% %     \right]^{-1}_{ }
% % \end{align*}
% % By computing the eigenvalues of this matrix, we obtain the degrees of the $k$ communities.  

% % At this point, it is easy to solve for $\pi$:
% % \begin{align*}
% %     \left[
% %     \begin{array}{ccc}
% %     1   &   1   &   1   \\
% %     d_1^{ }   &   d_2^{ }   &   d_3^{ }   \\
% %     d_1^{2}   &   d_2^{2}   &   d_3^{2}
% %     \end{array}
% %     \right]\left[
% %     \begin{array}{c}
% %     \pi_1^{ }   \\
% %     \pi_2^{ }   \\
% %     \pi_3^{ }
% %     \end{array}
% %     \right]=\left[
% %     \begin{array}{c}
% %     1   \\
% %     \Edge   \\
% %     \Wedge
% %     \end{array}
% %     \right]
% % \end{align*}





% \section{The Graphical Matrix Pencil Method}

% Graph homomorphism densities of stochastic block model $\SBM\big(\pi_k^{ }\kern1pt,\kern-1ptB_{k\kPrime}^{ }\big)$

% % \centering{
% \begin{center}
%     $\FeynmanDiagram{3}$
% \end{center}

% % }

% \begin{align}
% % \mathop{\text{\Large$\mathbb{E}$}}_{G\sim(\pi_k^{ },B_{k\kPrime}^{ })}\bigg[\kern-4pt\BirootedGlyph{1}{1}{2}{1}{1}\bigg] = \prod_{i=1}^{|V(g)|} \sum_{k_i^{ } = 1}^{K} \Big(\pi_{k_1^{ }}^{ }\pi_{k_2^{ }}^{ }\cdots\pi_{k_{6}^{ }}^{ }\Big) \Big(B_{k_1^{ }k_2^{ }}^{ }B_{k_2^{ }k_3^{ }}^{ }\cdots B_{k_{4}^{ }k_{6}^{ }}^{ }\Big)
% %\kern-4pt\BirootedGlyph[0.35]{1}{1}{1}{1}{1}
% \mathop{\underbrace{\mu\big(g\big)\Big|_{\SBM\big(\pi_k^{ },B_{k\kPrime}^{ }\big)}}}_{\substack{\text{homomorphism density}\\\text{$\mu$ of a subgraph $g$ in an}\\\text{SBM given by $\pi_k^{ }$ and $B_{k\kPrime}^{ }$}\\\text{with $K$ communities}}}%&= \prod_{i\in V(g)} \sum_{k_i^{ } = 1}^{K} \pi_{k_i^{ }}^{ } \prod_{(i\kern-1pt,\kern1pt j)\in E(g)}^{ } B_{k_i^{ }k_j^{ }}^{ }\nonumber\\
% &= \underbrace{\sum_{k_i^{ }: V_g^{ }\rightarrow[K]}^{|V_g^{ }|^K_{ }}}_{\substack{\text{sum over all maps}\\ \text{from vertices in $g$}\\ \text{to the $K$ communities}}} \Bigg[\underbrace{\Bigg(\prod_{i\in V_g^{ }} \kern-2pt \pi_{k_i^{ }}^{ }\Bigg)}_{\substack{\text{probability of that}\\\text{vertex assignment}}} \kern0pt\times\kern2pt \underbrace{\Bigg(\prod_{(i\kern-1pt,\kern1pt j)\in E_g^{ }}^{ } \kern-6pt B_{k_i^{ }k_j^{ }}^{ }\Bigg)}_{\substack{\text{probability of the}\\\text{corresponding edges}}}\Bigg]
% \nonumber
% \end{align}

% \begin{align}
% % \mathop{\text{\Large$\mathbb{E}$}}_{G\sim(\pi_k^{ },B_{k\kPrime}^{ })}\bigg[\kern-4pt\BirootedGlyph{1}{1}{2}{1}{1}\bigg] = \prod_{i=1}^{|V(g)|} \sum_{k_i^{ } = 1}^{K} \Big(\pi_{k_1^{ }}^{ }\pi_{k_2^{ }}^{ }\cdots\pi_{k_{6}^{ }}^{ }\Big) \Big(B_{k_1^{ }k_2^{ }}^{ }B_{k_2^{ }k_3^{ }}^{ }\cdots B_{k_{4}^{ }k_{6}^{ }}^{ }\Big)
% %\kern-4pt\BirootedGlyph[0.35]{1}{1}{1}{1}{1}
% \mathop{\underbrace{\mu\big(g_{r}^{ }\big)}}_{\substack{\text{homomorphism density}\\\text{$\mu$ of a rooted subgraph $g_{r}^{ }$}}}%&= \prod_{i\in V(g)} \sum_{k_i^{ } = 1}^{K} \pi_{k_i^{ }}^{ } \prod_{(i\kern-1pt,\kern1pt j)\in E(g)}^{ } B_{k_i^{ }k_j^{ }}^{ }\nonumber\\
% &= \underbrace{\sum_{k_i^{ }: V_g^{ }\setminus r\rightarrow[K]}^{|V_g^{ }\setminus r|^K_{ }}}_{\substack{\text{sum over all maps}\\ \text{from unrooted vertices}}} \kern-4pt\Bigg[\Bigg(\prod_{i\in V_g^{ }\setminus r} \kern-2pt \pi_{k_i^{ }}^{ }\Bigg) \kern0pt\times\kern2pt \Bigg(\prod_{(i\kern-1pt,\kern1pt j)\in E_g^{ }}^{ } \kern-6pt B_{k_i^{ }k_j^{ }}^{ }\Bigg)\Bigg]
% \nonumber
% \end{align}

% % \subsection{Notation}

% % \subsubsection{Tootsie-roll subgraphs}
% % % \label{ssec:tootsierollsubgraphs}
% % Union of the open neighborhood of two labelled nodes.  \\
% % We are exactly counting injective homomorphism densities.  \\
% % % We represent these subgraphs as a 3-tuple $((l),(c),(r))$, \\
% % % where $l$ is either $0$ or $1$ and 

% \begin{center}
% \begin{tabular}{ c l l }
%  glyph & symbol & meaning \\ 
%  \hline
%  \OpenNodeOld & $1_i^{ }$ & vector of ones of length $k$\\  
%  % \ClosedNodeOld & $\pi_i^{ }$ & vector of the $k$ community sizes \\  
%  \OpenNodeOldEdge & $d_i^{ } = W_{i\!j}^{ } \pi_j^{ }$ & vector of the $k$ normalized degrees  \\
%  \OpenNodeOldTwoEdge & $d_i^{2}$ & \\
%  \vdots 
% \end{tabular}
% \end{center}




% \begin{center}
% \begin{tabular}{ c l l }
%  glyph & definition & meaning \\ 
%  \hline
%  \ExampleTootsieRoll & see below & bilabelled tootise-roll graph\\
%  \OpenTwoNode & $\matt{1}_{i\!j}^{ } - \matt{I}_{i\!j}^{ }$ & matrix of ones on the off-diagonal\\  
%  \OpenTwoNodeCenterEdge & $\matt{W}_{i\!j}^{ }$ & matrix of edge probabilities \\  
%  \vdots 
% \end{tabular}
% \end{center}



% \begin{center}
% \begin{tabular}{ r c l }
% labelled node & $\longleftrightarrow$ & vector of ones \\
% gluing labelled nodes & $\longleftrightarrow$ & entrywise multiplication \\
% % closed node & $\longleftrightarrow$ & vector of community sizes \\
% % closing a node & $\longleftrightarrow$ & entrywise multiplication by community sizes \\
% unlabelling a labelled node & $\longleftrightarrow$ & summing over communities \\
% \end{tabular}
% \end{center}




% \subsection{Extracting the Edge Expectations}
% The previous matrices $M$ and $M'$ were obtained by summing once over the $k$ communities.  This allowed us to obtain properties related to a single community (eg, the degree $d_i^{ }$).  
% To obtain properties related to a pair of communities (ie, the connection probability $w_{i\!j}^{ }$), the sum must be over such pairs.  
% Notice that the matrices being summed in Equation %~\eqref{Eq:MDegreeOuterProductSum} 
% are outer the outer product of two vectors of length $k$, containing the powers of the degree of that community.  
% In this section, we do the same with a vector that contains the symmetric polynomials in the two degrees of the communities in question.  For an SBM with $2$ communities, this would be:
% \begin{align}
%     M_{i\!j}^{ } &= \sum_{k,\ell}^{ } \pi_k^{ }\pi_{\ell}^{ }
%     \left[
%     \begin{array}{c}
%     1   \\
%     \half{d_k^{ }+d_{\ell}^{ }}   \\
%     d_k^{ }d_{\ell}^{ }   
%     \end{array}
%     \right]
%     \left[
%     \begin{array}{ccc}
%     1   &   \half{d_k^{ }+d_{\ell}^{ }}   &   d_k^{ }d_{\ell}^{ }   
%     \end{array}
%     \right]\nonumber\\
%     &=\sum_{k,\ell}^{ } \pi_k^{ }\pi_{\ell}^{ }
%     \left[
%     \begin{array}{ccc}
%     1   &   \half{d_k^{ }+d_{\ell}^{ }}   &   d_k^{ }d_{\ell}^{ }   \\
%     \half{d_k^{ }+d_{\ell}^{ }}   &    \half{\half{d_k^{2}+d_{\ell}^{2}}+d_k^{ }d_{\ell}^{ }}   &   \half{d_k^{2}d_{\ell}^{ }+d_k^{ }d_{\ell}^{2}}   \\
%     d_k^{ }d_{\ell}^{ }     &       \half{d_k^{2}d_{\ell}^{ }+d_k^{ }d_{\ell}^{2}} &   d_k^{2}d_{\ell}^{2}
%     \end{array}
%     \right]
%     \label{Eq:MWOuterProductSum}
% \end{align}
% This matrix can be constructed by observable subgraph densities:
% \begin{align*}
%     M_{i\!j}^{ } = \left[
%     \begin{array}{ccc}
%     1   &   \Edge   &   \EdgeEdge   \\
%     \Edge   &   \half{\Wedge+\EdgeEdge}   &   \EdgeWedge   \\
%     \EdgeEdge   &   \EdgeWedge   &   \Wedge\;\!\Wedge
%     \end{array}
%     \right]
% \end{align*}
% and can also be decomposed into a diagonal matrix between two ``Vandermonde'' matrices:
% \begin{align*}
%     M_{i\!j}^{ }=\left[
%     \begin{array}{ccc}
%     1   &   1   &   1   \\
%     d_1^{ }   &   \half{d_1^{ }+d_{2}^{ }}   &   d_2^{ }   \\
%     d_1^{2}   &   d_1^{ }d_{2}^{ }   &   d_2^{2}   
%     \end{array}
%     \right]\left[
%     \begin{array}{ccc}
%     \pi_1^{2}   &   0   &   0   \\
%     0   &   2\pi_1^{ }\pi_2^{ }   &   0   \\
%     0   &   0   &   \pi_2^{2}
%     \end{array}
%     \right]\left[
%     \begin{array}{ccc}
%     1   &   d_1^{ }   &   d_1^{2}   \\
%     1   &   \half{d_1^{ }+d_{2}^{ }}   &   d_1^{ }d_{2}^{ }   \\
%     1   &   d_2^{ }   &   d_2^{2}   
%     \end{array}
%     \right]
% \end{align*}

% Now, to construct the analogous $M'$, we multiply every term in the sum in Equation~\eqref{Eq:MWOuterProductSum} by $w_{k\ell}^{ }$:
% \begin{align}
%     M'_{i\!j} &= \sum_{k,\ell}^{ } \pi_k^{ }\pi_{\ell}^{ }w_{k\ell}^{ }
%     \left[
%     \begin{array}{ccc}
%     1   &   \half{d_k^{ }+d_{\ell}^{ }}   &   d_k^{ }d_{\ell}^{ }   \\
%     \half{d_k^{ }+d_{\ell}^{ }}   &    \half{\half{d_k^{2}+d_{\ell}^{2}}+d_k^{ }d_{\ell}^{ }}   &   \half{d_k^{2}d_{\ell}^{ }+d_k^{ }d_{\ell}^{2}}   \\
%     d_k^{ }d_{\ell}^{ }     &       \half{d_k^{2}d_{\ell}^{ }+d_k^{ }d_{\ell}^{2}} &   d_k^{2}d_{\ell}^{2}
%     \end{array}
%     \right]
%     \label{Eq:MPrimeWOuterProductSum}
% \end{align}
% In terms of observable subgraph densities:
% \begin{align*}
%     M'_{i\!j} = \left[
%     \begin{array}{ccc}
%     \Edge   &   \Wedge   &   \Line   \\
%     \Wedge   &   \half{\Claw+\Line}   &   \BistarOneTwo   \\
%     \Line   &   \BistarOneTwo   &   \BistarTwoTwo
%     \end{array}
%     \right]
% \end{align*}
% and in terms of the decomposition:
% \begin{align*}
%     M'_{i\!j}=\left[
%     \begin{array}{ccc}
%     1   &   1   &   1   \\
%     d_1^{ }   &   \half{d_1^{ }+d_{2}^{ }}   &   d_2^{ }   \\
%     d_1^{2}   &   d_1^{ }d_{2}^{ }   &   d_2^{2}   
%     \end{array}
%     \right]\left[
%     \begin{array}{ccc}
%     \pi_1^{2}w_{11}^{ }   &   0   &   0   \\
%     0   &   2\pi_1^{ }\pi_2^{ }w_{12}^{ }   &   0   \\
%     0   &   0   &   \pi_2^{2}w_{22}^{ }
%     \end{array}
%     \right]\left[
%     \begin{array}{ccc}
%     1   &   d_1^{ }   &   d_1^{2}   \\
%     1   &   \half{d_1^{ }+d_{2}^{ }}   &   d_1^{ }d_{2}^{ }   \\
%     1   &   d_2^{ }   &   d_2^{2}   
%     \end{array}
%     \right]
% \end{align*}

% As before, the second matrix times the inverse of the first is
% \begin{align*}
%     M'_{ }M^{-1}_{ } = \left[
%     \begin{array}{ccc}
%     1   &   1   &   1   \\
%     d_1^{ }   &   \half{d_1^{ }+d_{2}^{ }}   &   d_2^{ }   \\
%     d_1^{2}   &   d_1^{ }d_{2}^{ }   &   d_2^{2}   
%     \end{array}
%     \right]\left[
%     \begin{array}{ccc}
%     w_{11}^{ }   &   0   &   0   \\
%     0   &   w_{12}^{ }   &   0   \\
%     0   &   0   &   w_{22}^{ }
%     \end{array}
%     \right]\left[
%     \begin{array}{ccc}
%     1   &   d_1^{ }   &   d_1^{2}   \\
%     1   &   \half{d_1^{ }+d_{2}^{ }}   &   d_1^{ }d_{2}^{ }   \\
%     1   &   d_2^{ }   &   d_2^{2}   
%     \end{array}
%     \right]^{-1}_{ }
% \end{align*}
% However, different than before, we can extract the entries of $W$ one by one.  
% The eigenvectors associated to each are simply the rows in the last matrix.  
% So to get $w_{i\!j}^{ }$, one would estimate the eigenvalue of its corresponding eigenvector: 
% \begin{align*}
%     w_{i\!j}^{ } = \frac{v^\intercal_{ }(M'_{ }M^{-1}_{ })v}{v^\intercal_{ }v}\\
%     v = \left[
%     \begin{array}{c}
%     1   \\
%     \half{d_i^{ }+d_{j}^{ }}   \\
%     d_i^{ }d_{j}^{ }   
%     \end{array}
%     \right]
% \end{align*}

% % \subsection{Matrix with More Moments}
% \subsection{Adding more subgraph densities}

% \begin{align*}
%     M_{i\!j}^{ } = \left[
%     \begin{array}{cccc}
%     1   &   \Edge   &   \Wedge   &   \Claw   \\
%     \Edge   &   \Wedge   &   \Claw   &   \Cross
%     \end{array}
%     \right]
% \end{align*}

% \begin{align*}
%     M'_{i\!j} = \left[
%     \begin{array}{cccc}
%     \Edge   &   \Wedge   &   \Claw   &   \Cross \\
%     \Wedge   &   \Claw   &   \Cross  &   \FiveStar
%     \end{array}
%     \right]
% \end{align*}

% \begin{align}
%     M_{i\!j}^{ } = \sum_k^{ } \pi_k^{ }
%     \left[
%     \begin{array}{cccc}
%     d_k^{0}   &   d_k^{1}   &   d_k^{2}   &   d_k^{3}   \\
%     d_k^{1}   &   d_k^{2}   &   d_k^{3}   &   d_k^{4}
%     \end{array}
%     \right]
%     \label{Eq:MExtraDegreeOuterProductSum}
% \end{align}

% \begin{align*}
%     \left[
%     \begin{array}{cc}
%     1   &   1   \\
%     d_1^{ }   &   d_2^{ }   
%     \end{array}
%     \right]\left[
%     \begin{array}{cc}
%     \pi_1^{ }   &   0   \\
%     0   &   \pi_2^{ }   
%     \end{array}
%     \right]\left[
%     \begin{array}{cccc}
%     1   &   d_1^{ }   &   d_1^{2}   &   d_1^{3}   \\
%     1   &   d_2^{ }   &   d_2^{2}   &   d_2^{3}   
%     \end{array}
%     \right]
% \end{align*}

% \begin{align*}
%     M'_{ }M^{\dagger}_{ } = \left[
%     \begin{array}{cc}
%     1   &   1   \\
%     d_1^{ }   &   d_2^{ }   
%     \end{array}
%     \right]\left[
%     \begin{array}{cc}
%     d_1^{ }   &   0   \\
%     0   &   d_2^{ }   
%     \end{array}
%     \right]\left[
%     \begin{array}{cc}
%     1   &   d_1^{ }   \\
%     1   &   d_2^{ }   
%     \end{array}
%     \right]^{-1}_{ }
% \end{align*}


% \newpage

% \section{Applying the Graphical Matrix Pencil Method to Observed Data} 
% \label{sec:ApplyingToData}

% \section{Efficiently counting the relevant subgraphs} 
% \label{sec:subgraphcount}



% % \newpage
% \subsection{Obtaining their (injective homomorphism) counts}
% \label{ssec:tootsierollcounts}


% We start with the adjacency matrix $\matt{A}_{i\!j}^{ }$, the identity matrix $\matt{I}_{i\!j}^{ }$, and the all-ones matrix $\matt{1}_{i\!j}^{ }$.  
% Then, we perform our only difficult matrix multiplication: 
% \mbox{\(\sum_k^{ }\matt{A}_{ik}^{ }\matt{A}_{kj}^{ } = \twohop_{i\!j}^{ } + \matt{D}_{i\!j}^{ }\)}, 
% where $\matt{D}_{i\!j}^{ }$ is the diagonal matrix of node degrees, and $\twohop_{i\!j}^{ }$ is the (traceless) ``two-hop adjacency'' matrix.  

% We will use $\bullet$ to denote matrix multiplication and $\circ$ for entrywise (Hadamard) multiplication: 
% \begin{align}
% \big(\matt{B} \bullet \matt{C}\big)_{i\!j}^{ } &= \sum_k^{ }\matt{B}_{ik}^{ }\matt{C}_{kj}^{ }\\
% \big(\matt{B} \circ \matt{C}\big)_{i\!j}^{ } &= \matt{B}_{i\!j}^{ }\matt{C}_{i\!j}^{ }
% \end{align}
% We use these operations to construct various matrices corresponding to (bi)rooted subgraph counts.  
% To obtain the subgraph counts in the entire graph, we will ``unroot'' them by taking the sum of all entries: 
% \begin{align}
% \llbracket \matt{Z} \rrbracket &= \sum_i^{ }\sum_j^{ }\matt{Z}_{i\!j}^{ }
% \end{align}
% For example, \mbox{$\llbracket \matt{A} \rrbracket$} is twice the number of edges, as the injective homomorphisms count both orientations.  

% \subsubsection{Star subgraphs}
% % Define a matrix of ``left degrees'': \mbox{\(\matt{L} = \matt{D}\bullet\big(\matt{1}-\matt{I}\big) - \matt{A}\)}, 
% % i.e., when \mbox{$i\neq j$}, the degree of node $i$ if node $j$ were deleted, and zero when \mbox{$i = j$}.  
% The injective homomorphism counts of the the $k$-star subgraphs \mbox{$K_{1,k}^{ }$} (i.e., containing one node adjacent to $k$ others) are given recursively: 
% \begin{align}
%     % c_{ }^{\text{(inj,hom)}}
%     \numsymbol\big(K_{1,k}^{ }\big) &= 
%     \Big\llbracket \matt{M}_{K_{1,k}^{ }}^{ } \Big\rrbracket\\
%     \matt{M}_{K_{1,1}^{ }}^{ } &= \matt{D}\\
%     \matt{M}_{K_{1,k+1}^{ }}^{ } &= \matt{M}_{K_{1,k}^{ }}^{ } \circ \big( \matt{D} - k\matt{I} \big) 
%     % \matt{M}_{K_{1,k+1}^{ }}^{ } &= \matt{M}_{K_{1,k}^{ }}^{ } \circ \big( \matt{L} - (k-1)\matt{1} \big) 
% \end{align}
% The counts of the ``tootsie-roll'' subgraphs can likewise be computed recursively.  

% \subsubsection{``Double-star'' subgraphs}
% The recursion begins with constructing matrices for (bipartite) subgraphs \mbox{$K_{2,k}^{ }$}, with two nodes that are adjacent to $k$ others: 
% \begin{align}
%     \matt{M}_{K_{2,1}^{ }}^{ } &= \twohop\\
%     \matt{M}_{K_{2,k+1}^{ }}^{ } &= \matt{M}_{K_{2,k}^{ }}^{ } \circ \big( \twohop - k\matt{1} \big) 
% \end{align}
% The entries of these matrices count the number of these subgraphs for which the two nodes are $i$ and $j$.  
% Thus, by multiplying by $A$, we get matrices for the ``double-star'' subgraphs \mbox{$K_{2,k}^{+}$}, with two nodes connected to $k$ others as well as each other.  
% \begin{align}    
%     \matt{M}_{K_{2+,k}^{ }}^{ } &= \matt{M}_{K_{2,k}^{ }}^{ } \circ \matt{A}
% \end{align}
% From these matrices, we obtain the counts as before: \mbox{$\numsymbol(g) = \llbracket \matt{M}_g^{ } \rrbracket$}.  

% \subsubsection{``Tootsie-roll'' subgraphs}

% % \subsubsection{Tootsie-roll subgraphs}
% % \label{ssec:tootsierollsubgraphs}
% Union of the open neighborhood of two labelled nodes.  \\
% We are exactly counting injective homomorphism densities.  \\
% % We represent these subgraphs as a 3-tuple $((l),(c),(r))$, \\
% % where $l$ is either $0$ or $1$ and 


% We will index our subgraphs with a tuple of non-negative integers \mbox{$(\ell,c,r)$}, corresponding to: 
% the number of single edges on the ``left'' node $i$, the number of 2-paths connected node $i$ and node $j$, and the number of single edges on the ``right'' node $j$.  
% First, we add the 2-paths:
% \begin{align}
%     \matt{M}_{(0,0,0)}^{ } &= \matt{1} - \matt{I}\\
%     \matt{M}_{(0,c+1,0)}^{ } &= \matt{M}_{(0,c,0)}^{ } \circ \big( \twohop - c \matt{1} \big)\\
%     % \matt{M}_{(0,c',0)}^{ } &= \matt{M}_{(0,c,0)}^{ } \circ \matt{A}
% \end{align}
% Define the matrix of ``left'' degrees to be \mbox{$\matt{L} = \matt{D}\bullet\matt{M}_{(0,0,0)}^{ } - \matt{A}$} (i.e., 
% %$ = \matt{R}^{\!\top}_{ }$}.\footnote{e.g., for $\matt{L}$, , when \mbox{$i\neq j$}
% the degree of node $i$ if node \mbox{$j\neq i$} were deleted, and zero when \mbox{$i = j$}), and the matrix of ``right'' degrees to be its transpose \mbox{$\matt{R} = \matt{L}^{\!\top}$}.  
% Next, we add single edges to node $i$, then to node $j$:
% \begin{align}
%     \matt{M}_{(\ell+1,c,0)}^{ } &= \matt{M}_{(\ell,c,0)}^{ } \circ \big( \matt{L} - (\ell+c) \matt{1}\big)\\
%     \matt{M}_{(\ell,c,r+1)}^{ } &= \matt{M}_{(\ell,c,r)}^{ } \circ \big( \matt{R} - (r+c) \matt{1}\big) - \ell\matt{M}_{(\ell-1,c+1,r-1)}^{ }
% \end{align}
% Finally, if an edge connecting node $i$ and $j$ is to be included, we put a mark on the middle integer: 
% \begin{align}
%     \matt{M}_{(\ell,c',r)}^{ } &= \matt{M}_{(\ell,c,r)}^{ } \circ \matt{A}
% \end{align}



% \newpage

% \begin{itemize}
%     \item Counting the statistics contained in a pair of open 1-neighborhoods, 
%     loop over all pairs of nodes %, watch out for integer overflows
% \end{itemize}

% \begin{itemize}
%     \item Explain the method for obtaining the injective homomorphism counts of the tootsie-roll subgraphs 
% \end{itemize}

\appendix




% \section{Improving the Matrix Pencil} 

% \subsection{Scaling by the precision} 

% \subsubsection{Estimating the variance} 
% \label{ssec:variance}
% We can estimate this using a sort of jackknife estimator.  
% In contrast to typical implementations, we can do this without incurring additional computational cost.  
% For each node, we can count the number of injective homomorphism counts are removed if that node were deleted.  
% Then we can use the distribution of these counts to estimate the variance of that subgraph density:
% \begin{align}
%     \mathrm{Var}\big(\mu_g^{ }(G)\big) \approx \frac{n}{n-1}\sum_{i=1}^n \Big(\mu_g^{ }(G\setminus i) - \mu_g^{ }(G) \Big)^{\kern-1pt2}_{ }
% \end{align}
% For each node, we already have the number of counts for which it is one of the center nodes of the subgraph.  
% For the counts where it is one of the neighboring nodes, 
% we can use the same ideas as before, computing the estimator exactly without increasing computational cost.  

% To verify the correctness of these expressions, 
% we take a generic SBM and simulate multiple graphs with $n$ nodes, 
% and compare the variance of the observed distribution of subgraph densities with the distribution of the estimated variances.  

% \begin{itemize}
%     \item Give an idea of the error in the approximation of the variance 
%     \item Give an idea of magnitude of the improvement 
%     % \item Discussion of what subgraphs to include
% \end{itemize}

% \subsection{Using more orthogonal linear combinations} 


% \section{Experiments}
% \subsection{Synthetic data}
% Convergence:
% \begin{itemize}
%     \item Toy problem: 2x2, equal communities, positive clustering, positive degree heterogeneity
%     \item Two curves per plot, one large degree separation, one small (maybe a third)
%     \item Plot accuracy of pentagon (square and triangle too?) density
%     \item As a function of number of nodes in the graph
%     \item Do one with constant edge density, one with constant expected degree
% \end{itemize}
% Parameter selection:
% \begin{itemize}
%     \item Same as above (but maybe with a 3x3)
%     \item Show convergence curves for k-1, k and k+1
% \end{itemize}

% \section{Discussion}
% \label{sec:Discussion}

% \paragraph{Future directions}

% \begin{itemize}
% % \item Using more orthogonal linear combinations (cumulantification)
% \item Extension to the case of communities with the same degree by exploiting the symmetries of the connectivity matrix 
%     \item Assigning nodes likelihoods of being particular communities, 
%     using node-typed moments to refine, leading to an E-M type algorithm (eg, \cite{ruffini2017hierarchical})
% \end{itemize}

    

% Maintext is 12 pages 



% \newpage
% \section{Motivation}
% \label{sec:Motivation}

% \paragraph{Inference in network models}
% % \label{ssec:RelatedWorkNetworks}
% \begin{itemize}
%     \item notoriously hard to do efficient inference in network models 
%     \item focus discussion on models that have subgraph densities as constrained statistics
%     \begin{itemize}
%         \item ERGMs --- list problems (degeneracy and approximating the partition function/convergence of MCMC type algorithms)
%         \item SBMs --- advantages 
%         \begin{itemize}
%             \item maximum entropy if disconnected subgraphs constrained to be equal the products (ie, single graphon assumption) with the caveat of being on the interior of the domain of graphonic possibilities
%             \item exchangeable over nodes for any $n$ and consistent nested distributions under node subsampling (ie, marginalizable)
%         \end{itemize} 
%         \item SBMs --- related work on inference
%         \begin{itemize}
%             \item spectral detection -- community detection -- sbm recovery -- focus on symmetric SBM case \cite{abbe2015detection,abbe2015community}
%             \item bayesian inference (tiago 
%             \cite{peixoto2014hierarchical}) -- iterative, computationally expensive 
%         \end{itemize}
%     \end{itemize}
% \end{itemize}

% \paragraph{Related work}

% \begin{itemize}
%     \item Variational Bayes model averaging for graphon functions and motif frequencies inference in W-graph models \cite{latouche2016variational}
% \end{itemize}

% \paragraph{Matrix pencil method}
% % \label{ssec:RelatedProny}
% \begin{itemize}
%    \item Method of moments 
%     \item Prony's method \cite{sauer2018prony, prony1795essai}
%     \item Renewed theoretical interest in this type of models -- eg, COLT2021 source identification for mixture of discrete product distributions \cite{gordon2021source} 
%     \item Matrix pencil 
%     \item Compressed sensing \cite{candes2006stable}
% \end{itemize}

% \newpage

% \noindent

% \section{Outline for the paper}
% \textbf{Motivation} \\[6pt]
% Inferring graph models from a single graph is nontrivial and currently and difficult \\[6pt]
% The principle of maximum entropy is a natural guide,\\
% but current methods with ERGMs frequently have problems with both inference and sampling \\[6pt]
% Fortunately, when the data is assumed to come from a single graphon,\\
% generic maximum entropy distributions have the structure of a block model \\[6pt]
% Introduce notation for the connectivity matrix $B_{ij}$\\and vector of community sizes $\pi_i$\\[6pt]
% Give outline of the paper:\\
% first describe the method for exact subgraph densities,\\
% then explain how to estimate from observed data\\[12pt]
% \textbf{Exact matrix pencil method} \\[6pt]
% Describe matrix pencil method for simple product distribution \\[-18pt]
% \begin{itemize}
%     \item coin flips from a distribution of coin biases $b_i$, each with probability $\pi_i$
%     \item define the Hankel matrix of moments $M$ and the shifted matrix $M'$
%     \item cite and state the answer: $\text{eigval}(M'M^{-1}) = b_i$
% \end{itemize}
% Getting the degree distribution is an exact application of this method \\[-18pt]
% \begin{itemize}
%     \item show why it works algebraically using $d_i$ and $\pi_i$ notation
% \end{itemize}
% Getting the connectivity matrix is an extension of this method \\[-18pt]
% \begin{itemize}
%     \item first insight --- applying matrix pencil to unordered pairs of latent variables
%     \item introduce glyph notation in table (open circle as labelled node, labelling and unlabelling operations)
%     \item show previous example with degrees using glyph notation
%     \item show how one can do the same eigenvalue trick to get the edge probabilities
%     \item but we don't know which probability goes where!
%     \item second insight --- we can leverage the inferred degrees of the communities to assign these eigenvalues to specific entries in $B_{ij}$ (briefly go back to algebraic notation for describing the eigenvectors, show equivalent representation in footnote)
% \end{itemize}


% \textbf{Inferring distribution from data} \\[6pt]
% Getting unbiased estimators \\[-18pt]
% \begin{itemize}  
%     \item briefly return to coin flip model, unbiased estimators of the moments are products of \textit{different} flips from the same coin
%     \item for graphs, the analogue is the \textit{injective} homomorphism densities
%     \item show how to recursively count the injective homomorphisms (for the ones we have seen so far ie,  stars and bi-stars), we need entrywise matrix multiplication 
%     \item because of injectivity, this naturally forces us to count subgraphs with two-edge paths between the labelled nodes
% \end{itemize}
% Tootsie-roll subgraphs \\[-18pt]
% \begin{itemize}    
%     \item  motivation:
%     \begin{itemize}
%         \item essentially, to infer the probability of an edge between two nodes, we use the intersection of the open neighborhoods of these two nodes, ie, all dyads that share a node with this (potential) edge 
%         \item we can count them fast using entrywise multiplication of $n\times n$ (with the overhead of a single matrix multiplication of the adjacency with itself)
%     \end{itemize}
%     \item introduce tuple notation, show recursion for counting injective homomorphisms
%     \item table of starting matrices and a few examples 
% \end{itemize}


% Adding additional subgraphs
% \begin{itemize}
%     \item But what happens when the degrees of two communities become similar?  % (but not to the point that the first step fails, the second one fails first -- community assigments contribute to larger fluctuations in the dense regime)
%     \item Since we have already been forced to count the density of general tootsie-roll subgraphs, we can actually leverage them to make the method more robust
%     \item By adding subgraphs with cycles to the matrices (making them rectangular and using pseudoinverse), we can better distinguish between communities with similar degrees 
% \end{itemize}
% Beyond Bickel % (when the degrees of the communities are exactly the same)
% \begin{itemize}
%     \item What if the degrees of the communities are exactly the same?  
%     \item The first step of getting the community degrees is meaningless beyond providing the edge density.  But we can use the eigenvalue method in the second step instead, to extract the entries of the connection matrix.  
%     \item Example with SSBM: the two eigenvalues are the inter- and intra-connection probabilities, from which we can infer the number of communities using the edge density
% \end{itemize}

\textbf{Main takeaway $\&$ Future directions}
\begin{itemize}
    \item The matrix pencil method can be applied to other representations of data
    \item It infers a plausible underlying model directly from summary statistics, without the need to work with the entirety of the observed data.  
    \item For graphs, it could be used as a tool for EM-type algorithms that aim to explicitly assign the observed nodes to inferred communities.  
\end{itemize}


% \textbf{Outline of method section COPY}

% \begin{enumerate}
%     \item Section outlining how this method section will go: 
%     \begin{itemize}
%       \item define goal of inferring a SBM
%       \begin{itemize}
%       \item giving the notation for the connectivity matrix $B_{ij}$ and vector of community sizes $\pi_i$
%       \item and making the distinction between using exact moments from a distribution and inferring the moments from an observed graph % data
%       \end{itemize}
%       \item now give the outline 
%        \begin{itemize}
%         \item first, we will explain how to get exact 
%         \item then, how to infer from data
%          \end{itemize}
%     \item to get exact, the sections go as following:
%     % \begin{itemize}
%     %     \item cite classical prony for mixture without proving
%     %     \item proving prony for degree distribution using standard algebraic notation
%     %     \item translate to single glyph notation
%     % \end{itemize}
%     \item to infer, the sections go as following:
%         % \begin{itemize}
%     %     \item cycles -- the idea has reach 
%     % \end{itemize}
%     \end{itemize}
% \item Recovering distribution using exact moments
%    \begin{itemize}
%     \item Matrix pencil method for simple product distribution %\textit{(with exact moments)}
%     \begin{itemize}
%         \item fast, cite, vector of coin biases b
%         \item define the Hankel matrix with moments $M$ and the shifted matrix $M'$
%     \end{itemize}
%     \item Getting the degree distribution %\textit{(with exact moments)}
%     \begin{itemize}
%         \item first step is essentially that method using degrees
%         \item show why it works algebraic (and using the stars glyphs) and why it is the mixture case with degrees 
%     \end{itemize}
%     \item Getting the connectivity matrix %\textit{(with exact moments)}
%     \begin{itemize}
%         \item first insight -- applying Prony to unordered pairs of latent variables
%         % ,\\
%         % and that, by construction, the eigenvectors are known based on the degrees (allowing for ordering these pairs) 
%         \item to make things clear, we will add a glyph notation
%         \item translate to single glyph notation the degree and the mixture model case
%         \begin{itemize}
%             \item open circle as labelled node, labelling and unlabelling operations
%         \end{itemize}
%          \item now getting the connectivity matrix:
%          \begin{itemize}
%              \item specify to communities with different degrees for now (Bickel-like assumption)
%              \item algebraically, we can do the same thing to the edge expectation as a (unordered) set (see appendix), but we will stick with the glyphs because they are more intuitive 
%              \item do concrete example with glyphs and show 2nd insight  -- ie, by construction, the eigenvectors are known based on the degrees, allowing for ordering the edge expectation (say algebraically and then glyphs)
%          \end{itemize}
%     \end{itemize}
%     \end{itemize}
%     \item Inferring distribution using from data
%     % \item Introducing tootsie-roll subgraphs 
%     % \begin{itemize}
%     %     \item motivations: 
%     %     \begin{itemize}
%     %         \item when communities have the same degree, cycles can help
%     %         \item when inferring injective homo is  unbiasing, forced to counting 2-path anyway
%     %         \item fast counting, nestedness
%     %         \item inference about proba of dyad between the nodes, open neighborhood 
%     %     \end{itemize}
%     % \end{itemize}
% \end{enumerate}



%%%%%%%%%%%%%%%%%%%%
% \begin{itemize}
%     \item Recovering distribution using exact moments
%     \begin{itemize}
%         \item Matrix pencil method for simple product distribution %\textit{(with exact moments)}
%         \begin{itemize}
%             \item fast, cite, vector of coin biases b
%             \item define the Hankel matrix with moments $M$ and the shifted matrix $M'$
%         \end{itemize}
%         \item Getting the degree distribution %\textit{(with exact moments)}
%         \begin{itemize}
%             \item first step is essentially that method using degrees
%             \item show why it works algebraic (and using the stars glyphs) and why it is the mixture case with degrees 
%         \end{itemize}
%         \item Getting the connectivity matrix %\textit{(with exact moments)}
%         \begin{itemize}
%             \item first insight -- applying Prony to unordered pairs of latent variables
%             % ,\\
%             % and that, by construction, the eigenvectors are known based on the degrees (allowing for ordering these pairs) 
%             \item to make things clear, we will add a glyph notation
%             \item translate to single glyph notation the degree and the mixture model case
%             \begin{itemize}
%                 \item open circle as labelled node, labelling and unlabelling operations
%             \end{itemize}
%             \item now getting the connectivity matrix:
%             \begin{itemize}
%                  \item specify to communities with different degrees for now (Bickel-like assumption)
%                  \item algebraically, we can do the same thing to the edge expectation as a (unordered) set (see appendix), but we will stick with the glyphs because they are more intuitive 
%                  \item do concrete example with glyphs and show 2nd insight  -- ie, by construction, the eigenvectors are known based on the degrees, allowing for ordering the edge expectation (say algebraically and then glyphs)
%              \end{itemize}
%         \end{itemize}
%     \end{itemize}
%     \item Inferring distribution from data
%     \begin{itemize}
%         \item briefly return to coin flip model, unbiased estimators of the moments are products of \textit{different} flips from the same coin
%         \item for graphs, the analogue is the \textit{injective} homomorphism densities
%         \item show how to recursively count the injective homomorphisms (for the ones we have seen so far ie,  stars and bi-stars), we need entrywise matrix multiplication 
%         \item because of injectivity, this naturally forces us to count subgraphs with two-edge paths between the labelled nodes
%         \item introduce tootsie-roll subgraphs, motivation:
%         \begin{itemize}
%             \item essentially, to infer the probability of an edge between two nodes, we use the intersection of the open neighborhoods of these two nodes, ie, all dyads that share a node with this (potential) edge 
%             \item we can count them fast using entrywise multiplication of $n\times n$ (with the overhead of a single matrix multiplication of the adjacency with itself)
%         \end{itemize}
%         \item introduce tuple notation, show recursion for counting injective homomorphisms
%         \item table of starting matrices and a few examples 
%         %
%         \item Adding additional subgraphs
%         \begin{itemize}
%             \item But what happens when the degrees of two communities become similar?  % (but not to the point that the first step fails, the second one fails first -- community assigments contribute to larger fluctuations in the dense regime)
%             \item Since we have already been forced to count the density of general tootsie-roll subgraphs, we can actually leverage them to make the method more robust
%             \item By adding subgraphs with cycles to the matrices (making them rectangular and using pseudoinverse), we can better distinguish between communities with similar degrees 
%         \end{itemize}
%         \item Beyond Bickel % (when the degrees of the communities are exactly the same)
%         \begin{itemize}
%             \item What if the degrees of the communities are exactly the same?  
%             \item The first step of getting the community degrees is meaningless beyond providing the edge density.  But we can use the eigenvalue method in the second step instead, to extract the entries of the connection matrix.  
%             \item Example with SSBM: the two eigenvalues are the inter- and intra-connection probabilities, from which we can infer the number of communities using the edge density
%         \end{itemize}
%     \end{itemize}
%     \item Main takeaway/Future directions
%     \begin{itemize}
%         \item The matrix pencil method can be applied to other representations of data
%         \item It infers a plausible underlying model directly from summary statistics, without the need to work with the entirety of the observed data.  
%         \item For graphs, it could be used as a tool for EM-type algorithms that aim to explicitly assign the observed nodes to inferred communities.  
%     \end{itemize}
% \end{itemize}


% % there are different ways the degrees of the communities can be the same, due to symmetries (the extreme example being k-ssbm) or no symmetries (coincidental, break in communities inside communities)


% \newpage

